Infinite-dimensional port-Hamiltonian systems with a stationary interface

We consider two systems of two conservation laws that are defined on complementary, one-dimensional spatial intervals and coupled by an interface as a single port-Hamiltonian system. In case of a fixed interface position, we characterize the boundary and interface conditions for which the associated port-Hamiltonian operator generates a contraction semigroup. Furthermore, we present sufficient conditions for the exponential stability of the generated $C_0$-semigroup. The results are illustrated by the example of two acoustic waveguides coupled by a membrane interface.

==> references.tex <==
@article{Aggelis_07,
    author = {Aggelis, D. G. and Shiotani, T.},
    title = {Experimental study of surface wave propagation in strongly heterogeneous media},
    journal = {The Journal of the Acoustical Society of America},
    volume = {122},
    number = {5},
    pages = {EL151-EL157},
    year = {2007},
    month = {09},
    issn = {0001-4966},
    doi = {10.1121/1.2784151}
}

@book{Visintin1996models,
  title={Models of {P}hase {T}ransitions},
  author={Visintin, A.},
  year={1996},
  edition={First},
  publisher={Springer Science \& Business Media},
 series={Progress in Nonlinear Differential Equations and Their Applications},
 volume={28}
}

@Article{Datko1968,
  author  = {R. Datko},
  journal = {Journal of Mathematical Analysis and Applications},
  title   = {An extension of a theorem of {A}. {M}. {L}yapunov to semigroup operators},
  year    = {1968},
  pages   = {290--295},
  volume  = {24},
}

@Book{Pazy1983,
  author    = {A. Pazy},
  publisher = {Springer, New York},
  title     = {Semigroups of {L}inear {O}perators and {A}pplications to {P}artial {D}ifferential {E}quations},
  year      = {1983},
  edition   = {First},
  isbn      = {0-387-90845-5},
  series    = {Applied Mathematical Sciences},
  volume    = {44},
}

@Article{Diagne2013,
  author  = {M. Diagne and B. M. Maschke},
  journal = {European Journal on Control},
  title   = {Port {H}amiltonian formulation of a system of two conservation laws with a moving interface},
  year    = {2013},
  number  = {6},
  pages   = {495--504},
  volume  = {19},
}

@Book{Jacob2012,
  author    = {B. Jacob and H. J. Zwart},
  publisher = {Birkhäuser/Springer Basel AG, Basel},
  title     = {Linear {P}ort-{H}amiltonian {S}ystems on {I}nfinite-dimensional {S}paces},
  year      = {2012},
  edition   = {First},
  isbn      = {978-3-0348-0398-4},
  series    = {Operator Theory: Advances and Applications},
  volume    = {223},
}

@Book{Engel2000,
  author    = {K.-J. Engel and R. Nagel},
  publisher = {Springer, New York},
  title     = {One-{P}arameter {S}emigroups for {L}inear {E}volution {E}quations},
  year      = {2000},
  edition   = {First},
  isbn      = {0-387-98463-1},
  series    = {Graduate Texts in Mathematics},
  volume    = {194},
}

@Article{Gorrec2005,
  author  = {Y. Le Gorrec and H. J. Zwart and B. M. Maschke},
  journal = {SIAM Journal on Control and Optimization},
  title   = {Dirac structures and boundary control systems associated with skew-symmetric differential operators},
  year    = {2005},
  number  = {5},
  pages   = {1864--1892},
  volume  = {44},
}

@Book{Aubin2000,
  author    = {J.-P. Aubin},
  publisher = {John Wiley \& Sons, New York},
  title     = {Applied {F}unctional {A}nalysis},
  year      = {2000},
  edition   = {Second},
  series    = {Wiley Series in Pure and Applied Mathematics},
}

@Article{Schaft2014,
  author  = {A. J. van der Schaft and D. Jeltsema},
  journal = {Foundations and Trends® in Systems and Control},
  title   = {Port-{H}amiltonian systems theory: an introductory overview},
  year    = {2014},
  number  = {2-3},
  pages   = {173--378},
  volume  = {1},
}

@PhdThesis{Villegas2007,
  author = {J. A. Villegas},
  school = {Department of Applied Mathematics, University of Twente, Enschede},
  title  = {A port-{H}amiltonian approach to distributed parameter systems},
  year   = {2007},
}

@MastersThesis{Kilian2022,
  author = {A. Kilian},
  school = {Chair of Dynamical Systems, University of Passau},
  title  = {Infinite-{D}imensional {P}ort-{H}amiltonian {S}ystems with a {M}oving {I}nterface},
  year   = {2022},
  eprint={2301.07344},
  archivePrefix={arXiv},
  primaryClass={math.AP},
  url={https://arxiv.org/abs/2301.07344}
}

@Book{Arnold1978,
  author    = {V. I. Arnol'd},
  publisher = {Springer, New York},
  title     = {Mathematical {M}ethods of {C}lassical {M}echanics},
  year      = {1978},
  series    = {Graduate Texts in Mathematics},
  volume    = {60},
}

@Book{Paynter1961,
  author    = {H. M. Paynter},
  publisher = {MIT Press, Cambridge, Massachusetts},
  title     = {Analysis and {D}esign of {E}ngineering {S}ystems},
  year      = {1961},
}

@Book{Curtain2020,
  author    = {R. F. Curtain and H. J. Zwart},
  publisher = {Springer, New York},
  title     = {Introduction to {I}nfinite-{D}imensional {L}inear {S}ystems {T}heroy},
  year      = {2020},
  edition   = {First},
  series    = {Texts in Applied Mathematics},
  volume    = {71},
}

@Book{Tucsnak2009,
  author    = {M. Tucsnak and G. Weiss},
  publisher = {Birkhäuser, Basel},
  title     = {Observation and {C}ontrol for {O}perator {S}emigroups},
  year      = {2009},
  edition   = {First},
  series    = {Birkhäuser Advanced Texts Basler Lehrbücher},
}

@PhdThesis{Augner2016,
  author = {B. Augner},
  school = {Department of Mathematics and Informatics, University of Wuppertal},
  title  = {Stabilisation of infinite-dimensional port-{H}amiltonian systems via dissipative boundary feedback},
  year   = {2016},
}

@Article{Fattorini1968,
  author  = {H. O. Fattorini},
  journal = {SIAM Journal on Control},
  title   = {Boundary control systems},
  year    = {1968},
  number  = {3},
  pages   = {349--385},
  volume  = {6},
}

@Book{Duindam2009,
  editor    = {V. Duindam and A. Macchelli and S. Stramigioli and H. Bruyninckx},
  publisher = {Springer, Berlin Heidelberg},
  title     = {Modeling and {C}ontrol of {C}omplex {P}hysical {S}ystems},
  year      = {2009},
  edition   = {First},
}

@Book{Gupta2003,
  author    = {S. C. Gupta},
  publisher = {Elsevier, Amsterdam},
  title     = {The {C}lassical {S}tefan {P}roblem},
  year      = {2003},
  edition   = {First},
  series    = {North-Holland Series in Applied Mathematics and Mechanics},
  volume    = {45},
}

@Article{Godlewski2004,
  author  = {E. Godlewski and P.-A. Raviart},
  journal = {Numer. Math.},
  title   = {The numerical interface coupling of nonlinear hyperbolic systems of conservation laws},
  year    = {2004},
  pages   = {81--130},
  volume  = {97},
}

@InProceedings{Boutin2008,
  author    = {B. Boutin and F. Coquel and E. Godlewski},
  booktitle = {Hyperbolic Problems: Theory, Numerics, Applications},
  title     = {Dafermos {R}egularization for {I}nterface {C}oupling of {C}onservation {L}aws},
  year      = {2008},
  editor    = {S. Benzoni-Gavage and D. Serre},
  pages     = {567--575},
  publisher = {Springer Berlin, Heidelberg},
}

@Article{CardosoRibeiro2017,
  author  = {F. L. Cardoso-Ribeiro and D. Matignon and V. Pommier-Budinger},
  journal = {Journal of Fluids and Structures},
  title   = {A port-{H}amiltonian model of liquid sloshing in moving containers and application to a fluid-structure system},
  year    = {2017},
  pages   = {402--427},
  volume  = {69},
}

@Article{Gorrec2017,
  author  = {Y. Le Gorrec and H. Zwart and H. Ramirez},
  journal = {IFAC-PapersOnLine},
  title   = {Asymptotic stability of an {E}uler-{B}ernoulli beam coupled to non-linear spring-damper systems},
  year    = {2017},
  number  = {1},
  pages   = {5580--5585},
  volume  = {50},
}

@Article{Hamroun2010,
  author  = {B. Hamroun and A. Dimofte and L. Lefèvre and E. Mendes},
  journal = {European Journal of Control},
  title   = {Control by interconnection and energy-shaping methods of port-{H}amiltonian models - {A}pplication to the shallow water equations},
  year    = {2010},
  number  = {5},
  pages   = {545--563},
  volume  = {16},
}

@Article{Kobayasi1979,
  author  = {K. Kobayasi},
  journal = {Journal of the Mathematical Society of Japan},
  title   = {On a theorem for linear evolution equations of hyperbolic type},
  year    = {1979},
  number  = {4},
  pages   = {647--654},
  volume  = {31},
}

@Article{Nickel1998,
  author  = {G. Nickel and R. Schnaubelt},
  journal = {Taiwanese Journal of Mathematics},
  title   = {An extension of {K}ato's stability condition for nonautonomous {C}auchy problems},
  year    = {1998},
  number  = {4},
  pages   = {483--496},
  volume  = {2},
}

@Book{Teschl2012,
  author    = {Gerald Teschl},
  publisher = {American Mathematical Society, Providence},
  title     = {Ordinary {D}ifferential {E}quations and {D}ynamical {S}ystems},
  year      = {2012},
  edition   = {First},
  series    = {Graduate Studies in Mathematics},
  volume    = {140},
}

@article{Kurula_IJC_15,
author = {Kurula,M. and Zwart,H.},
title = {Linear wave systems on n-D spatial domains},
journal = {International Journal of Control},
volume = {88},
number = {5},
pages = {1063-1077},
year  = {2015},
publisher = {Taylor & Francis},
mydoi = {10.1080/00207179.2014.993337},
myeprint = {https://doi.org/10.1080/00207179.2014.993337}
}

@ARTICLE{schaftGeomPhys02,
  author =    {A.J. van der Schaft and  B.M. Maschke},
  title =     {Hamiltonian formulation of distributed parameter systems with boundary energy flow},
  journal =   {J. of Geometry and Physics},
  year =      { 2002},
  volume =    {42},
  number =    {},
  pages =     {166-174},
  }

@book{Olver93,
	Address = {New-York},
	Author = {Olver, P.J.},
	Edition = {II},
	Note = {ISBN 0-387-94007-3},
	Publisher = {Springer},
	Series = {Graduate texts in mathematics},
	Title = {Applications of {L}ie Groups to {D}ifferential {E}quations},
	Volume = {107},
	Year = {1993}}

@article{Rashad_IMA18_20yearsBPHS,
    author = {Rashad, R.and Califano, F. and van der Schaft, A. and Stramigioli, S.},
    title = "{Twenty years of distributed port-Hamiltonian systems: a literature review}",
    journal = {IMA Journal of Mathematical Control and Information},
    year = {2020},
    month = {07},
    issn = {1471-6887},
    mydoi = {10.1093/imamci/dnaa018},
    myurl = {https://doi.org/10.1093/imamci/dnaa018},
    annote = {dnaa018},
    myeprint = {https://academic.oup.com/imamci/advance-article-pdf/doi/10.1093/imamci/dnaa018/33537885/dnaa018.pdf},
}

@article{Lotero_MCMDS17,
author = {Lotero, F.  and Couenne, F.  and Maschke,B.  and Sbarbaro, D. },
title = {Distributed parameter bi-zone model with moving interface of an extrusion process and experimental validation},
journal = {Mathematical and Computer Modelling of Dynamical Systems},
volume = {23},
number = {5},
pages = {504-522},
year = {2017},
mydoi = {10.1080/13873954.2016.1278393},
}
@article{Ogam_ApplAcoustics_21,
title = {Investigation of long acoustic waveguides for the very low frequency characterization of monolayer and stratified air-saturated poroelastic materials},
journal = {Applied Acoustics},
volume = {182},
pages = {108200},
year = {2021},
issn = {0003-682X},
mydoi = {https://doi.org/10.1016/j.apacoust.2021.108200},
myurl = {https://www.sciencedirect.com/science/article/pii/S0003682X21002942},
author = {Ogam, E. and El Abiddine Fellah, Z. and  Ogam, G. and Ongwen, N.O. and  Oduor, N.O.},
}

@article{Willatzen_IntJRefrigeration1998,
title = {A general dynamic simulation model for evaporators and condensers in refrigeration. {P}art {I}: {M}oving-boundary formulation of two-phase flows with heat exchange},
journal = {International Journal of Refrigeration},
volume = {21},
number = {5},
pages = {398-403},
year = {1998},
issn = {0140-7007},
mydoi = {https://doi.org/10.1016/S0140-7007(97)00091-1},
myurl = {https://www.sciencedirect.com/science/article/pii/S0140700797000911},
author = {M. Willatzen and N.B.O.L. Pettit and L. Ploug-S\"orensen},
}

@article{Jacob_JEvEq2015c,
  title={C 0-semigroups for hyperbolic partial differential equations on a one-dimensional spatial domain},
  author={Jacob, B. and Morris, K. and Zwart, H.},
  journal={Journal of Evolution Equations},
  volume={15},
  number={2},
  pages={493--502},
  year={2015},
  publisher={Springer}
}

@article{Kurula_JMAA_10,
title = "Dirac structures and their composition on {H}ilbert spaces",
journal = "Journal of Mathematical Analysis and Applications",
volume = "372",
number = "2",
pages = "402 - 422",
year = "2010",
issn = "0022-247X",
mydoi = "https://doi.org/10.1016/j.jmaa.2010.07.004",
author = "Kurula, M. and Zwart, H. and van der Schaft, A. and Behrndt, J.",
keywords = "Dirac structure, Composition, Boundary triplet, Boundary colligation, Impedance conservative, Kre?n space"
}

@article{Vincent_IFAC_WC20_PhaseFields,
  TITLE = {{Port {H}amiltonian systems with moving interface: a phase field approach}},
  AUTHOR = {Vincent, B. and Couenne, F. and Lef{\`e}vre, L. and Maschke, B.},
  journal = {IFAC-PapersOnLine},
volume = {53},
number = {2},
pages = {7569-7574},
year = {2020},
note = {21th IFAC World Congress},
issn = {2405-8963},
mydoi = {https://doi.org/10.1016/j.ifacol.2020.12.1353},
}

@ARTICLE{KMMW23,
  author={Kilian, Alexander and Maschke, Bernhard and Mironchenko, Andrii and Wirth, Fabian},
  journal={IEEE Control Systems Letters}, 
	title = {A case study of port-{H}amiltonian systems with a moving interface},
  year={2023},
  volume={7},
  number={},
  pages={1572-1577},
  citeulike-linkout-0 = {http://arxiv.org/abs/2302.03344},
	citeulike-linkout-1 = {https://ieeexplore.ieee.org/document/10113681?source=authoralert}
}

@Comment{jabref-meta: databaseType:bibtex;}


@InProceedings{Augner2020,
author="Augner, Bj{\"o}rn",
editor="Kerner, Joachim
and Laasri, Hafida
and Mugnolo, Delio",
title="Well-posedness and stability for interconnection structures of port-{H}amiltonian type",
booktitle="Control Theory of Infinite-Dimensional Systems",
year="2020",
publisher="Springer International Publishing",
address="Cham",
pages="1--52"
}

